Evaluating the Effectiveness of Retrieval-Augmented Large Language Models in Scientific Document Reasoning

Despite the dramatic progress in Large Language Model (LLM) development, LLMs often provide seemingly plausible but not factual information, often referred to as hallucinations. Retrieval-augmented LLMs provide a non-parametric approach to solve these issues by retrieving relevant information from external data sources and augment the training process. These models help to trace evidence from an externally provided knowledge base allowing the model predictions to be better interpreted and verified. In this work, we critically evaluate these models in their ability to perform in scientific document reasoning tasks. To this end, we tuned multiple such model variants with science-focused instructions and evaluated them on a scientific document reasoning benchmark for the usefulness of the retrieved document passages. Our findings suggest that models justify predictions in science tasks with fabricated evidence and leveraging scientific corpus as pretraining data does not alleviate the risk of evidence fabrication.

==> backup/notes.tex <==
\shnote{
The big question: how can we provide more information to help people critically assess AI outputs and make better decisions, without biasing them towards trusting the AI?
background explanations also increase people's confidence even when models are wrong~\cite{goyal2023else}
Trust in the Absence of Verifiability: Consider asking ChatGPT to explain its answer to a reading comprehension question. What it would say would probably make sense on the surface. Ditto with a saliency map explaining a visual model. But this doesn't verify the answer, ie wedon't know if the model is correct.}

==> backup/rq2.tex <==
\section{Improving Evidence Extraction with Scientific Knowledge Guiders}

Does improving the relevance and diversity of the generated evidence increase the science tasks performance? 

\paragraph{SciGuide helps reducing the scientific evidence fabrication}

\paragraph{SciGuide increases the accuracy of in- and out-of-distribution science-focused tasks}



